Characterization and Mitigation of ADC Noise by Reference Tuning in RRAM-Based Compute-In-Memory

With the escalating demand for power-efficient neural network architectures, non-volatile compute-in-memory designs have garnered significant attention. However, owing to the nature of analog computation, susceptibility to noise remains a critical concern. This study confronts this challenge by introducing a detailed model that incorporates noise factors arising from both ADCs and RRAM devices. The experimental data is derived from a 40nm foundry RRAM test-chip, wherein different reference voltage configurations are applied, each tailored to its respective module. The mean and standard deviation values of HRS and LRS cells are derived through a randomized vector, forming the foundation for noise simulation within our analytical framework. Additionally, the study examines the read-disturb effects, shedding light on the potential for accuracy deterioration in neural networks due to extended exposure to high-voltage stress. This phenomenon is mitigated through the proposed low-voltage read mode. Leveraging our derived comprehensive fault model from the RRAM test-chip, we evaluate CIM noise impact on both supervised learning (time-independent) and reinforcement learning (time-dependent) tasks, and demonstrate the effectiveness of reference tuning to mitigate noise impacts.

==> tabs/table_example.tex <==
\begin{table}[t!]
\centering
\vspace{-5pt}
\caption{Comparison of fault injection techniques at various layers of abstraction. Software-level approach is adopted in our experiments.}
\vspace{-3pt}
\renewcommand*{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Abstraction}\\ \textbf{Layer} \end{tabular} & \textbf{Platform}                                                                 & \begin{tabular}[c]{@{}c@{}}\textbf{Perf.}\\ \textbf{(cycles/sec)} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Drone E2E Exec.}\\ \textbf{Time (1 run)} \end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{Drone E2E Exec.}\\ \textbf{Time (1000 runs)} \end{tabular} \\ \hline

RTL                  & \begin{tabular}[c]{@{}c@{}}IVM processor\\ RTL simulation~\cite{maniatakos2010instruction} \end{tabular} & 6$\times$$10^2$     & 2.5$\times$$10^{5}$ hours               & 1.04$\times$$10^{7}$days                 \\ \hline 

Micro-architecture         & gem5 simulator~\cite{binkert2011gem5}                                                                    & 3$\times$$10^6$     & 50.0 hours                 & 2083 days                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FPGA Emulation \end{tabular}   & \begin{tabular}[c]{@{}c@{}}OpenSPARC T1\\ FPGA emulation~\cite{pellegrini2012crashtest} \end{tabular}                                                     & 1$\times$$10^7$     & 15 hours                   & 624 days                     \\ \hline

Architecture               & TSIM simulator~\cite{danvek2013leon3}                                                              & 6$\times$$10^7$     & 2.50 hours                 & 104.2 days                    \\ \hline



\textbf{Software (Ours)}            & \textbf{CPU processor} ~\cite{yim2010measurement}                                                                     & \textbf{3$\mathbf{\times 10^9}$}     & \textbf{3 mins}                     & \textbf{2.09 days}                    \\ \hline

\end{tabular}
}
\label{tab:FI_compare}
\vspace{-5pt}
\end{table}

